SWIFT: Super-fast and Robust Privacy-Preserving Machine Learning

Performing machine learning (ML) computation on private data while maintaining data privacy, aka Privacy-preserving Machine Learning~(PPML), is an emergent field of research. Recently, PPML has seen a visible shift towards the adoption of the Secure Outsourced Computation~(SOC) paradigm due to the heavy computation that it entails. In the SOC paradigm, computation is outsourced to a set of powerful and specially equipped servers that provide service on a pay-per-use basis. In this work, we propose SWIFT, a robust PPML framework for a range of ML algorithms in SOC setting, that guarantees output delivery to the users irrespective of any adversarial behaviour. Robustness, a highly desirable feature, evokes user participation without the fear of denial of service. At the heart of our framework lies a highly-efficient, maliciously-secure, three-party computation (3PC) over rings that provides guaranteed output delivery (GOD) in the honest-majority setting. To the best of our knowledge, SWIFT is the first robust and efficient PPML framework in the 3PC setting. SWIFT is as fast as (and is strictly better in some cases than) the best-known 3PC framework BLAZE (Patra et al. NDSS'20), which only achieves fairness. We extend our 3PC framework for four parties (4PC). In this regime, SWIFT is as fast as the best known fair 4PC framework Trident (Chaudhari et al. NDSS'20) and twice faster than the best-known robust 4PC framework FLASH (Byali et al. PETS'20). We demonstrate our framework's practical relevance by benchmarking popular ML algorithms such as Logistic Regression and deep Neural Networks such as VGG16 and LeNet, both over a 64-bit ring in a WAN setting. For deep NN, our results testify to our claims that we provide improved security guarantee while incurring no additional overhead for 3PC and obtaining 2x improvement for 4PC.

==> Main_4_PrivML.tex <==
In this section, we provide details regarding robust constructions of some of the widely used building blocks in PPML. This include i) Dot Product, ii) Truncation, iii) Dot Product with Truncation, iv) Secure Comparison , and v) Non-linear Activation functions-- Sigmoid and ReLU.



%------------------------------------------------------------------------------------------------------
\paragraph{Dot Product}
%------------------------------------------------------------------------------------------------------
Given the $\shrd$-sharing of vectors $\vecX$ and $\vecY$, protocol $\piDotP$ (\boxref{fig:piDotP}) allows servers to generate $\shrd$-sharing of $\vecX \band \vecY$ in a robust fashion. By $\shrd$-sharing of a vector $\vecX$ of size $\nf$, we mean that each element $\vx_i \in \Z{\ell}$ in the vector, for $i \in [\nf]$, is $\shrd$-shared. The dot product $\vecX \band \vecY$ can be viewed as $\nf$ parallel multiplication instances of the form $\wx_i \wy_i$ followed by adding up the results.  We modify the protocol for dot product as in BLAZE in a way that allows us to exploit $\piJmp$ to ensure GOD. 

During the preprocessing phase, servers execute the preprocessing corresponding to each of the $\nf$ multiplications ($\piMult$) of the form $\wz_i = \wx_i \wy_i$. Recall that the preprocessing of $\piMult$ requires a communication of $4$ ring elements and hence the preprocessing cost of $\piDotP$ will become $4\nf$ ring elements. We now show an optimization to bring this down to $3\nf +1$ ring elements. During the preprocessing for $\wz_i = \wx_i \wy_i$, recall that one ring element is communicated corresponding to $\Delta_i$ value that enables $P_0$ to readjust his shares for $\Gamma_{\wx_i\wy_i}$. We now show a method to club these $\Delta_i$'s so that a single element needs to be communicated. Towards this, $\ESet$ locally computes $\Delta = \sum_{i=1}^{\n} \Delta_i$ and sends this to $P_0$ using $\piJmp$ protocol. $P_0$ now readjusts his shares as $\sqr{\Gammaxy}_1 = \sum_{i=1}^{\n} \sqr{\GammaV{\wx_{i}\wy_{i}}}_1' + \Delta$ and $\sqr{\Gammaxy}_2 = \sum_{i=1}^{\n} \sqr{\GammaV{\wx_{i}\wy_{i}}}_2' - \Delta$.

During the online phase, following a naive solution would require servers to compute $\bv{\wz_i}$ for $i \in [\nf]$ first followed by computing $\bv{\wz} = \bv{{\wz}_1} + \ldots + \bv{{\wz}_\nf}$. Since this would result in a communication cost dependent on $\nf$, we use the idea of BLAZE to locally compute $\sqr{\bv{\wz}} = \sqr{\bv{{\wz}_1}} + \ldots + \sqr{\bv{{\wz}_\nf}}$ and reconstruct $\bv{\wz}$. Concretely, $P_0,P_1$ locally compute $\sqrV{\starbeta{\wz}}{1} = -\sum_{i=1}^{\nf} (\bv{\wx_i}+\gv{\wx_i})\sqrV{\av{\wy_i}}{1} - \sum_{i=1}^{\nf} (\bv{\wy_i}+\gv{\wy_i})\sqrV{\av{\wx_i} }{1}+ \sqrV{\av{\wz} }{1}+ 2\sqrV{\Gammaxy}{1} + \sqrV{\Chi}{1}$ and execute $\piJmp$ to enable $P_2$ to correctly reconstruct $\starbeta{\wz} = \sqrV{\starbeta{\wz}}{1} + \sqrV{\starbeta{\wz}}{2}$. In a similar fashion, $P_0, P_2$ computes and sends $\sqrV{\starbeta{\wz}}{2}$ to $P_1$ who computes $\starbeta{\wz}$. Finally, $\ESet$ locally compute $\bv{\wz}+\gv{\wz}$ and execute $\piJmp$ to enable $P_0$ obtain $\bv{\wz}+\gv{\wz}$. We defer the formal details of $\piDotP$ to Appendix~\ref{appsec:piDotP}.

%------------------------------------------------------------------------------------------------------
\paragraph{Truncation}
%------------------------------------------------------------------------------------------------------
Working over floating point values, repeated multiplications using FPA arithmetic can lead to an overflow resulting in loss of significant bits of information. This put forth the need for truncation~\cite{MohasselZ17,MR18,ASTRA,FLASH,BLAZE} that re-adjusts the shares after multiplication so that FPA semantics is maintained. As shown in SecureML~\cite{MohasselZ17}, the method of truncation would result in loss of information on the least significant bits and affect the accuracy by a very minimal amount only. 

For truncation, servers execute $\piTrunc$ (\boxref{fig:piTr}) to generate a random pair of the form $(\sqr{\vr}, \shr{\vrt})$. Here, $\vr$ denotes a random ring element, while $\vrt$ represents the truncated value of $\vr$. By truncated value, we mean that the value is right-shifted by $d$ bit positions, where $d$ is the number of bits allocated for the fractional part in the FPA representation. Given $(\vr, \vrt)$, the truncated value of $\val$ denoted by $\trunc{\val}$ can be computed from $\val$ as $\trunc{\val} = \trunc{(\val - \vr)} + \vrt$. As shown in ABY3~\cite{MR18}, this method ensures the same correctness of SecureML and the accuracy is affected by a very minimal amount.

To generate $(\sqr{\vr}, \shr{\vrt})$, servers proceed as follows: $P_0, P_j$ for $j \in \EInSet$ sample random $R_j \in \Z{\ell}$. $P_0$ locally computes $\vr = R_1 + R_2$ and truncates $\vr$ to obtain $\vrt$. $P_0$ then executes $\piSh$ on $\vrt$ to generate $\shr{\vrt}$. As shown in BLAZE, the correctness of sharing performed by $P_0$ is checked using the relation $\vr = 2^d \vrt + \vrd$,  where $\vrd$ denotes the ring element $\vr$ with the higher order $\ell - d$ bit positions set to $0$. In detail, $P_0, P_j$ for $j \in \{1,2\}$ locally computes $\sqr{\va_j}$ for $\va = (\vr - 2^d \vrt + \vrd)$. $P_0, P_1$ then sends $\Hash(\sqr{\va}_1)$ to $P_2$ using $\piJmp$ protocol. $P_2$ checks if the received hash value matches with $\Hash(-\sqr{\va}_2)$. In case of any inconsistency, $P_2$ accuses $P_0$ and then $P_1$ is identified as the TTP. The correctness of $\piTrunc$ follows trivially from BLAZE.

%-------------------
%Special pbox since this is not having any algohead in the beginning 
%-------------------
\begin{mypbox}{$\piTrunc(\Partyset)$}{Generating Random Truncated Pair $(\vr, \vrt)$}{fig:piTr}
	%-----
	\justify	
	\begin{myitemize}
		%-----
		\item[--] $P_0, P_j$ for $j \in \EInSet$ together sample random $R_j \in \Z{\ell}$. $P_0$ sets $\vr = R_1 + R_2$ while $P_j$ sets $\sqr{\vr}_{j} = R_j$. $P_j$ sets $\sqr{\vrd}_{j}$ as the ring element that has last $d$ bits of $\vr_j$ in the last $d$ positions and $0$ elsewhere.	
		%-----	
		\item[--] $P_0$ truncates $\vr$ to obtain $\vrt$ and executes $\piSh(P_0,\vrt)$ to generate $\shr{\vrt}$. 
		%-----	
		\item[--] $P_0,P_1$ set $\sqrA{\vrt} = \bv{\vrt}-\sqr{\av{\vrt}}_{1}$, while $P_0,P_2$ set $\sqrB{\vrt} =-\sqr{\av{\vrt}}_{2}$.
		%----
		\item[--] $P_0,P_1$ compute $\vu = \sqr{\vr}_{1} - 2^d \sqr{\vrt}_{1} - \sqr{\vrd}_{1}$. Servers in $\Partyset$ execute $\piJmp(P_0,P_1,P_2,\Hash(\vu))$ to enable $P_2$ obtain $\Hash(\vu)$. 
		%----
		\item[--] $P_2$ locally computes $\vv = 2^d \sqr{\vrt}_{2} + \sqr{\vrd}_{2} - \sqr{\vr}_{2}$. If $\Hash(\vu) \ne \Hash(\vv)$, $P_2$ $\broadcast$ \texttt{"accuse $P_0$"} and $P_1$ is chosen as the TTP.
		%----
		\item[--] If a TTP is identified in any of the protocol steps, TTP computes $(\sqr{\vr}, \shr{\vrt})$ and distributes among the servers. 
		%----
	\end{myitemize}  
\end{mypbox}
%-------------------
%\vspace{-3mm}

%------------------------------------------------------------------------------------------------------
\paragraph{Dot Product with Truncation}
%------------------------------------------------------------------------------------------------------
Given the $\shrd$-sharing of vectors $\vecX$ and $\vecY$, protocol $\piDotPTr$ (\boxref{fig:piDotPTr}) allows servers to generate $\shr{\trunc{\wz}}$, where $\trunc{\wz}$ denotes the truncated value of $\wz = \vecX \band \vecY$. One naive way is to compute the dot product using $\piDotP$ first, followed by performing the truncation using the $(\vr, \vrt)$ pair. Instead, we follow the optimization of BLAZE where the online phase of $\piDotP$ is modified to integrate the truncation using $(\vr, \vrt)$ at no additional cost.

The preprocessing phase now consists of the execution of one instance of $\piTrunc$ (\boxref{fig:piTr}) and the preprocessing corresponding to $\piDotP$ (\boxref{fig:piDotP}). At a high level, the online phase proceeds as follows: $P_0, P_j$ for $j \in \{1,2\}$ locally compute $\sqr{\wz^\star-\vr}_j$ (instead of $\sqr{\starbeta{\wz}}_j$ as in $\piDotP$) where $\wz^\star = \starbeta{\wz} - \av{\wz}$. Using $\piJmp$ protocol, $P_0,P_1$ sends $\sqr{\wz^\star-\vr}_1$ to $P_2$ while $P_0,P_2$ sends $\sqr{\wz^\star-\vr}_2$ to $P_1$. Both $\ESet$ then computes $(\wz - \vr)$ locally, truncates it to obtain $\trunc{(\wz-\vr)}$ and executes $\piJSh$ to generate $\shr{\trunc{(\wz-\vr)}}$. Finally, servers locally compute the result as $\shr{\trunc{\wz}} = \shr{\trunc{(\wz-\vr)}} + \shr{\vrt}$. We defer the formal details of the protocol $\piDotPTr$ to Appendix~\ref{appsec:piDotPTr}.

%------------------------------------------------------------------------------------------------------
\paragraph{Secure Comparison}
%------------------------------------------------------------------------------------------------------
Secure comparison allows servers to check whether $\wx < \wy$ or not, given their $\shrd$-shares. In FPA representation,  checking $\wx < \wy$ is equivalent to checking the $\MSB$ of $\val = \wx - \wy$. Towards this, servers locally compute $\shr{\val} = \shr{\wx} - \shr{\wy}$ and extract the $\MSB$ of $\val$ using $\piBitExt$ (\boxref{fig:piBitExt}). In case an arithmetic sharing is desired, servers can apply $\PiBitA$ (\boxref{fig:piBit2A}) protocol on the outcome of $\piBitExt$ protocol.

%------------------------------------------------------------------------------------------------------
\paragraph{Activation Functions}
%------------------------------------------------------------------------------------------------------
We now elaborate on the two of the most prominently used activation functions: i) Rectified Linear Unit (ReLU) and (ii) Sigmoid (Sig).

%-----------------------------------------
{\em -- ReLU:}
%-----------------------------------------
The ReLU function, $\ReLU(\val) = \maxv(0, \val)$, can be viewed as $\ReLU(\val) = \overline{\bitb} \cdot \val$, where the bit $\bitb = 1$ if $\val < 0$ and $0$ otherwise. Here $\overline{\bitb}$ denotes the complement of $\bitb$. 
%
Given $\shr{\val}$, servers first execute $\piBitExt$ on $\shr{\val}$ to generate $\shrB{\bitb}$. The $\shr{\cdot}$-sharing of $\overline{\bitb}$ is then locally computed by setting $\bv{\overline{\bitb}} = 1 \xor \bv{\bitb}$. Servers then execute $\PiBitInj$ protocol on $\shrB{\overline{\bitb}}$ and $\shr{\val}$ to obtain the desired result.

%-----------------------------------------
{\em -- Sig:}
%-----------------------------------------
In this work, we use the MPC-friendly variant of the Sigmoid function~\cite{MohasselZ17, MR18, ASTRA} as given below:
%-------------
\begin{align*}
	\Sig(\val) = \left\{
	\begin{array}{lll}
		0                  & \quad \val < -\frac{1}{2} \\
		\val + \frac{1}{2} & \quad - \frac{1}{2} \leq \val \leq \frac{1}{2} \\
		1                  & \quad \val > \frac{1}{2}
	\end{array}
	\right.
\end{align*}
%------------

Note that $\Sig(\val) = \overline{\bitb_1} \bitb_2 (\val + 1/2) + \overline{\bitb_2}$, where $\bitb_1 = 1$ if $\val + 1/2 < 0$ and $\bitb_2 = 1$ if $\val - 1/2 < 0$. To compute $\shr{\Sig(\val)}$, servers proceed in a similar fashion as the ReLU, and hence, we skip the formal details.

==> Main_5_Biometric.tex <==
Biometric computation is central to many real world tasks such as face recognition, genome sequence comparison, and fingerprint-matching\commentM{citations for the same}. The objective is, given a database $\DB$ of $m$ biometric samples stored as vectors $(\vecV{s}{1},\ldots,\vecV{s}{m})$, and a user with its own sample $\vecU$, identify the "closest" sample to $\vecU$ in $D$. \commentM{Do I have to cite earlier works here?} This task can be accomplished by considering various distance metrics, most prominent of which is the Euclidean distance. In this work we consider Euclidean distance as the metric, and hence the problem boils down to: identifying a sample vector in $D$ which has the least Euclidean distance with respect to $\vecU$.  Note that, in our setting, each entry in the database $\DB$ is shared among the servers in $\Partyset$. The client with an input query $\vecU$, generates $\shrd$- shares of the same along with the servers. 

Let $x_i$ denote the ith element in the vector $\vecX$. Euclidean distance between two n length vectors $\vecX$, $\vecY$ is computed as $\ED{\vecX}{\vecY} = \sum_{i=1}^{i=n}(x_i-y_i)^2$. This can be viewed as the dot product of the vector $\vecZ = ((x_1-y_1),\ldots,(x_n,y_n))$ with itself. Hence, $\ED{\vecX}{\vecY}$ is obtained by first computing $\shrd$-shares for vector $\vecZ$ locally, as $\shr{z_i} = \shr{x_i}-\shr{y_i}$ for $i \in [n]$, followed by an execution of $\piDotP$ on $\shr{\vecZ},\shr{\vecZ}$. For biometric computation, the servers, given $\shrd$-shares of $\vecU$, create a distance vector $\DV$ by computing the euclidean distance between $\vecU$ and every sample vector in $\DB$, i.e\ $\DV_i = \ED{\vecU}{\vecV{s}{i}}$ for $i \in [m]$.
 

The next task now is to find the minimum value in $\DV$. Minimum between two elements $a$, $b$ can be computed by applying secure comparison, which returns a binary sharing of a bit $c$ such that $c= 0$ if $a>b$, or 1, otherwise. The minimum of $a, b$ can be computed as $(c)^{\bf B}(a-b)+b$, which can be computed using bit injection (\secref{3PC}).
%As was shown in \cite{Trident}, XOR operation can be rewritten so that the above expression becomes: \commentN{Fill in the blank}. 
To find the minimum element in $\DV$, the servers first divides the elements of $\DV$ into pairs and securely compare each pair and obtain the minimum of the two, which results in a vector of size $m / 2$. This is repeated for $\BigO{\log(n)}$ rounds to obtain the minimum value, and consequently the closest $\vecV{s}{i} \in \DB$ to $\vecU$.



  




==> mintree.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt 
%\resizebox{.45\textwidth}{!}{
\begin{figure}[htb!]
	\resizebox{.8\textwidth}{!}{
	%----------------------------------------------------
	\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,167); %set diagram left start at 0, and has height of 167
	
	%Shape: Circle [id:dp01075325650516712] 
	\draw   (3.67,39) .. controls (3.67,29.98) and (10.98,22.67) .. (20,22.67) .. controls (29.02,22.67) and (36.33,29.98) .. (36.33,39) .. controls (36.33,48.02) and (29.02,55.33) .. (20,55.33) .. controls (10.98,55.33) and (3.67,48.02) .. (3.67,39) -- cycle ;
	%Straight Lines [id:da9227063140960146] 
	\draw    (20,55.33) -- (43.41,73.12) ;
	\draw [shift={(45,74.33)}, rotate = 217.23] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	
	%Straight Lines [id:da1032384596878424] 
	\draw    (70.33,55.33) -- (46.6,73.13) ;
	\draw [shift={(45,74.33)}, rotate = 323.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	
	%Straight Lines [id:da33770337060079103] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (191,69.33) -- (218.33,69.33) ;
	
	
	%Shape: Circle [id:dp2451762075508812] 
	\draw   (54,39) .. controls (54,29.98) and (61.31,22.67) .. (70.33,22.67) .. controls (79.35,22.67) and (86.67,29.98) .. (86.67,39) .. controls (86.67,48.02) and (79.35,55.33) .. (70.33,55.33) .. controls (61.31,55.33) and (54,48.02) .. (54,39) -- cycle ;
	%Shape: Circle [id:dp8075176364784626] 
	\draw   (104,39) .. controls (104,29.98) and (111.31,22.67) .. (120.33,22.67) .. controls (129.35,22.67) and (136.67,29.98) .. (136.67,39) .. controls (136.67,48.02) and (129.35,55.33) .. (120.33,55.33) .. controls (111.31,55.33) and (104,48.02) .. (104,39) -- cycle ;
	%Shape: Circle [id:dp5149937905768347] 
	\draw   (154.67,39.67) .. controls (154.67,30.65) and (161.98,23.33) .. (171,23.33) .. controls (180.02,23.33) and (187.33,30.65) .. (187.33,39.67) .. controls (187.33,48.69) and (180.02,56) .. (171,56) .. controls (161.98,56) and (154.67,48.69) .. (154.67,39.67) -- cycle ;
	%Shape: Circle [id:dp3123750287060161] 
	\draw   (224,40.67) .. controls (224,31.65) and (231.31,24.33) .. (240.33,24.33) .. controls (249.35,24.33) and (256.67,31.65) .. (256.67,40.67) .. controls (256.67,49.69) and (249.35,57) .. (240.33,57) .. controls (231.31,57) and (224,49.69) .. (224,40.67) -- cycle ;
	%Shape: Circle [id:dp9676973925968197] 
	\draw   (274.67,41.33) .. controls (274.67,32.31) and (281.98,25) .. (291,25) .. controls (300.02,25) and (307.33,32.31) .. (307.33,41.33) .. controls (307.33,50.35) and (300.02,57.67) .. (291,57.67) .. controls (281.98,57.67) and (274.67,50.35) .. (274.67,41.33) -- cycle ;
	%Shape: Circle [id:dp9649258103310128] 
	\draw   (28.67,90.67) .. controls (28.67,81.65) and (35.98,74.33) .. (45,74.33) .. controls (54.02,74.33) and (61.33,81.65) .. (61.33,90.67) .. controls (61.33,99.69) and (54.02,107) .. (45,107) .. controls (35.98,107) and (28.67,99.69) .. (28.67,90.67) -- cycle ;
	%Straight Lines [id:da6668272234681702] 
	\draw    (120.33,55.33) -- (143.39,72.47) ;
	\draw [shift={(145,73.67)}, rotate = 216.62] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	
	%Straight Lines [id:da8269432233886902] 
	\draw    (171,56) -- (146.65,72.54) ;
	\draw [shift={(145,73.67)}, rotate = 325.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	
	%Shape: Circle [id:dp6154091230363448] 
	\draw   (128.67,90) .. controls (128.67,80.98) and (135.98,73.67) .. (145,73.67) .. controls (154.02,73.67) and (161.33,80.98) .. (161.33,90) .. controls (161.33,99.02) and (154.02,106.33) .. (145,106.33) .. controls (135.98,106.33) and (128.67,99.02) .. (128.67,90) -- cycle ;
	%Straight Lines [id:da3290590669683149] 
	\draw    (240.33,57) -- (263.32,71.91) ;
	\draw [shift={(265,73)}, rotate = 212.97] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	
	%Straight Lines [id:da42127879201736596] 
	\draw    (291,57.67) -- (266.72,71.98) ;
	\draw [shift={(265,73)}, rotate = 329.47] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	
	%Shape: Circle [id:dp4208882247813861] 
	\draw   (248.67,89.33) .. controls (248.67,80.31) and (255.98,73) .. (265,73) .. controls (274.02,73) and (281.33,80.31) .. (281.33,89.33) .. controls (281.33,98.35) and (274.02,105.67) .. (265,105.67) .. controls (255.98,105.67) and (248.67,98.35) .. (248.67,89.33) -- cycle ;
	
	% Text Node
	\draw (20,39) node  [font=\normalsize]  {$\wx_{1}$};
	% Text Node
	\draw (70.33,39) node  [font=\normalsize]  {$\wx_{2}$};
	% Text Node
	\draw (45,90.67) node  [font=\normalsize]  {$\wy_{1}$};
	% Text Node
	\draw (120.33,39) node  [font=\normalsize]  {$\wx_{3}$};
	% Text Node
	\draw (171,39.67) node  [font=\normalsize]  {$\wx_{4}$};
	% Text Node
	\draw (240.33,40.67) node  [font=\normalsize]  {$\wx_{m-1}$};
	% Text Node
	\draw (291,41.33) node  [font=\normalsize]  {$\wx_{m}$};
	% Text Node
	\draw (145,90) node  [font=\normalsize]  {$\wy_{2}$};
	% Text Node
	\draw (265,89.33) node  [font=\normalsize]  {$\wy_{m/2}$};
	\end{tikzpicture}
	%----------------------------------------------------
	}
	\caption{Minimum Value - An example}
	\vspace{-3mm}
\end{figure}
%}

==> symbols.tex <==
%-----------------------------
%Math Symbols
%-----------------------------
\input{symbols/symbols_maths}

%-----------------------------
%Environments Symbols
%-----------------------------
\input{symbols/symbols_env_usenix}

%-----------------------------
%Circuit Symbols
%-----------------------------
\input{symbols/symbols_ckt}

%-----------------------------
%MPC Symbols
%-----------------------------
\input{symbols/symbols_mpc}

%-----------------------------
%BLAZE Symbols
%-----------------------------
\input{symbols/symbols_blaze}

%-----------------------------
%SWIFT 3PC Symbols
%-----------------------------
\input{symbols/symbols_3pc_SWIFT}

%-----------------------------
%SWIFT 4PC Symbols
%-----------------------------
\input{symbols/symbols_4pc_SWIFT}

%-----------------------------
%Biometric Symbols
\input{symbols/symbols_biometric}
%-----------------------------

==> symbols_env_ndss.tex <==
%To remove the left indentation of description environment
\setlist[description]{style=unboxed,leftmargin=0cm}

\newcommand{\myparagraph}[1]{\vspace{0.7em} \noindent \textbf{#1}}

%--------------------------------------------------------------
%Itemize, Enumerate, Description with less space
%--------------------------------------------------------------
\newenvironment{myitemize}{
	\begin{list}{{$\bullet$}}{
			\setlength\partopsep{0pt}
			\setlength\parskip{0pt}
			\setlength\parsep{0pt}
			\setlength\topsep{2pt}
			%\setlength\itemsep{3pt}
			\setlength\itemsep{2pt}
			\setlength{\itemindent}{0pt}
			\setlength{\leftmargin}{6pt}
		}
	}{
	%\vspace{1mm}
	\end{list}
}

\newenvironment{myitem}
{\setcounter{itemcount}{0}\begin{list}
		%{\arabic{itemcount}.}{
		%{\textbf{\arabic{itemcount}.}}{
		{\textbf{\arabic{itemcount})}}{
			\usecounter{itemcount} 
			\itemindent=4pt
			\itemsep=3pt
			\parskip=0pt
			\parsep=0pt
			\partopsep=0pt
			\topsep=2pt
			\partopsep=0.0in
			\leftmargin=3pt
			\labelindent=30pt
			\labelwidth=-1pt
	}}{\end{list}}



\newenvironment{newitemize}{
	\begin{list}{{$\bullet$}}{
			\setlength\partopsep{0pt}
			\setlength\parskip{0pt}
			\setlength\parsep{0pt}
			\setlength\topsep{2pt}
			\setlength\itemsep{4pt}
			\setlength{\itemindent}{1pt}
			\setlength{\leftmargin}{9pt}
		}
	}{
		%\vspace{1mm}
	\end{list}
}

\newenvironment{inneritemize}{
	\begin{list}{{$\bullet$}}{
			\setlength\partopsep{0pt}
			\setlength\parskip{0pt}
			\setlength\parsep{0pt}
			\setlength\topsep{2pt}
			\setlength\itemsep{2pt}
			\setlength{\itemindent}{2pt}
			\setlength{\leftmargin}{9pt}
		}
	}{
		%\vspace{0.1mm}
	\end{list}
}

\newenvironment{mylist}{
	\begin{list}{{$\bullet$}}{
			\setlength\partopsep{0pt}
			\setlength\parskip{0pt}
			\setlength\parsep{0pt}
			\setlength\topsep{2pt}
			\setlength\itemsep{1pt}
			\setlength{\itemindent}{0pt}
			\setlength{\leftmargin}{9pt}
		}
	}{
		%\vspace{0.1mm}
	\end{list}
}

\newenvironment{myenumerate}
{\setcounter{itemcount}{0}\begin{list}
{\arabic{itemcount}.}{
	\usecounter{itemcount} 
	\itemindent=-0.5cm
	\itemsep=0.0in
	\parsep=0.0in
	\topsep=0pt
	\partopsep=0.0in
}}{\end{list}}

\newenvironment{newenumerate}
{\setcounter{itemcount}{0}\begin{list}
		{\arabic{itemcount}.}{
			\usecounter{itemcount} 
			\itemindent=0cm
			\itemsep=3pt
			\parsep=0.0in
			\topsep=0pt
			\partopsep=0.0in
	}}{\end{list}}

\newlist{myenumlist}{enumerate}{2}
\setlist[myenumlist]{leftmargin=*,label={\arabic*)}}

\newenvironment{mydescription}
{\setcounter{itemcount}{0}\begin{list}
{\arabic{itemcount}.}{\usecounter{itemcount} \itemindent=-0.5cm
\itemsep=0.0in
\parsep=0.0in
\topsep=5pt
\partopsep=0.0in}}{\end{list}}

%------------------Not used----------------------------
\newenvironment{myitemizeold}
{\begin{list}{$\bullet$}{ %\itemindent=-.3cm \listparindent=.6cm
			\itemindent=-0.1in
			\itemsep=0.0in
			\parsep=0.0in
			\topsep=0.0in
			\partopsep=0.0in}}{\end{list}}
\newcounter{itemcount}

\newenvironment{compactlist}{
	\begin{list}{{$\bullet$}}{
			\setlength\partopsep{0pt}
			\setlength\parskip{0pt}
			\setlength\parsep{0pt}
			\setlength\topsep{0pt}
			\setlength\itemsep{0pt}
			\setlength{\itemindent}{0.4pt}
			\setlength{\leftmargin}{10pt}
		}
	}{
	\end{list}
}
%------------------Not used----------------------------

%--------------------------------------------------------------
%Commands for figures and tables and references
%--------------------------------------------------------------

\newcommand{\tabref}[1]{Table~\protect\ref{tab:#1}}
\newcommand{\secref}[1]{Section~\protect\ref{sec:#1}}
\newcommand{\lemref}[1]{Lemma~\protect\ref{lem:#1}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figlab}[1]{\label{fig:#1}}
\newcommand{\refeqn}[1]{Equation~\eqref{#1}}

\newenvironment{boxfig}[2]{% {#1}{#2} = {Caption}{label}
	\begin{figure}[ht!]
		\newcommand{\FigCaption}{#1}
		\newcommand{\FigLabel}{#2}
		\vspace{-.15cm}
		\begin{center}
			\begin{small}
				\begin{tabular}{@{}|@{~~}l@{~~}|@{}}
					\hline
					%\rule[-1ex]{0pt}{1ex}\begin{minipage}[!htb]{\textwidth}   
					\rule[-1.5ex]{0pt}{1ex}\begin{minipage}[b]{.97\linewidth}
						\vspace{1ex}
						\smallskip
					}{%
					\end{minipage}\\
					\hline
				\end{tabular}
			\end{small}
			\vspace{-0.3cm}
			\caption{\FigCaption}
			\figlab{\FigLabel}
		\end{center}
		\vspace{-0.4cm}
	\end{figure}
}


\newenvironment{boxfig*}[2]{% {#1}{#2} = {Caption}{label}
	\begin{figure*}[h!]		
		\fontsize{5}{5}\selectfont
		\newcommand{\FigCaption}{#1}
		\newcommand{\FigLabel}{#2}
		\vspace{-.05cm}
		\begin{center}
			\begin{small}			 
				\begin{adjustbox}{max width=\textwidth}
					\begin{tabular}{@{}|@{~~}l@{~~}|@{}}
						\hline
						%\rule[-1ex]{0pt}{1ex}\begin{minipage}[!htb]{\textwidth}   
						\rule[-1ex]{0pt}{1ex}\begin{minipage}[b]{.95\linewidth}
							\vspace{1ex}	
						}{%
						\end{minipage}\\
						\hline
					\end{tabular}	
				\end{adjustbox}		
			\end{small}
			\vspace{-0.1cm}
			\caption{\FigCaption}
			\figlab{\FigLabel}
		\end{center}
		\vspace{-.38cm}
	\end{figure*}
}

\newenvironment{myboxfig}[2]{% {#1}{#2} = {Caption}{label}
	\vspace{-0.5cm}
	\begin{figure}[htb!]		
		\fontsize{5}{5}\selectfont
		\newcommand{\FigCaption}{#1}
		\newcommand{\FigLabel}{#2}
		\vspace{-.15cm}
		\begin{center}
			\caption{\FigCaption}
			\begin{small}			 
				\begin{adjustbox}{max width=\textwidth}
					\begin{tabular}{@{}|@{~~}l@{~~}|@{}}
						\hline
						%\rule[-1ex]{0pt}{1ex}\begin{minipage}[!htb]{\textwidth}   
						\rule[-1ex]{0pt}{1ex}\begin{minipage}[b]{.95\linewidth}
							\vspace{1ex}	
						}{%
						\end{minipage}\\
						\hline
					\end{tabular}	
				\end{adjustbox}		
			\end{small}
			%	\vspace{-0.25cm}
			\figlab{\FigLabel}
		\end{center}
		\vspace{-.38cm}
	\end{figure}
}


\newenvironment{myboxfig*}[2]{% {#1}{#2} = {Caption}{label}
	\begin{figure*}[!htb]		
		\fontsize{5}{5}\selectfont
		\newcommand{\FigCaption}{#1}
		\newcommand{\FigLabel}{#2}
		\vspace{-.10cm}
		\begin{center}
			\caption{\FigCaption}
			\begin{small}			 
				\begin{adjustbox}{max width=\textwidth}
					\begin{tabular}{@{}|@{~~}l@{~~}|@{}}
						\hline
						%\rule[-1ex]{0pt}{1ex}\begin{minipage}[!htb]{\textwidth}   
						\rule[-1ex]{0pt}{1ex}\begin{minipage}[b]{.95\linewidth}
							\vspace{1ex}	
						}{%
						\end{minipage}\\
						\hline
					\end{tabular}	
				\end{adjustbox}		
			\end{small}
			\vspace{-0.25cm}
			\figlab{\FigLabel}
		\end{center}
		\vspace{-.38cm}
	\end{figure*}
}





%--------------------------------------------------------------
%New Style boxes
%--------------------------------------------------------------

%\newcommand{\boxref}[1]{Fig.~\ref{#1}}
\newcommand{\boxref}[1]{Fig. \ref{#1}}

%----- Box Environment ---------------------------------------------------------
\RequirePackage{mdframed}

%Basic box structure with title box
\newenvironment{titlebox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.1\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1.5em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	%\medskip
	\vspace{-2mm}
}

%title box style
\tikzstyle{normal} = [thick, fill=white, text=black, draw, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]
\tikzstyle{gray} = [thick, fill=gray!90, text=white, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]

%box style
\mdfdefinestyle{commonbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - 
	%innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
	%splittopskip=15pt,splitbottomskip=15pt
}


\mdfdefinestyle{roundbox}{style=commonbox,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{systembox}[3]
{\begin{titlebox}{Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{gsystembox}[3]
{\vspace{\baselineskip}\begin{titlebox}{Global Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{protocolbox}[3]
{\begin{titlebox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}


\newenvironment{algobox}[3]
{\begin{titlebox}{Algorithm \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{reductionbox}[3]
{\begin{titlebox}{Reduction \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{gamebox}[3]
{\begin{titlebox}{Game \normalfont #1}{commonbox}{gray}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{simulatorbox}[3]
{\begin{titlebox}{Simulator \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}
%-------------------------------------------------------------------------------



%-------------------------------------------------------------------------------
%Split Box for IEETran Version
%-------------------------------------------------------------------------------
%Basic box structure with title box
\newenvironment{splittitlebox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.1\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-0.5em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	%\medskip
	\vspace{-2mm}
}

\mdfdefinestyle{commonsplitbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - 
	%innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
	%splittopskip=15pt,splitbottomskip=15pt
}

\newenvironment{protocolsplitbox}[3]
{\begin{splittitlebox}{Protocol \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}

%------------------------------------------------------------------------------
% Full Width Environments
%------------------------------------------------------------------------------

\newenvironment{systembox*}[3]
{\begin{strip}
\vspace{\baselineskip}\begin{titlebox}{Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{gsystembox*}[3]
{\begin{strip}
\vspace{\baselineskip}\begin{titlebox}{Global Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{protocolbox*}[3]
{\begin{strip}
\begin{titlebox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{algobox*}[3]
{\begin{strip}
\begin{titlebox}{Algorithm \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{reductionbox*}[3]
{\begin{strip}
\begin{titlebox}{Reduction \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{gamebox*}[3]
{\begin{strip}
\begin{titlebox}{Game \normalfont #1}{commonbox}{gray}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{simulatorbox*}[3]
{\begin{strip}
\begin{titlebox}{Simulator \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}




%------------------------------------------------------------------------------
%Basic box structure with mytitle box without embossed title
%------------------------------------------------------------------------------

%box style
\mdfdefinestyle{mycommonbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=3pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
}
\mdfdefinestyle{myroundbox}{style=mycommonbox,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{titlebox*}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=0.3\baselineskip,
		skipabove={0.4em},
		skipbelow={1em},needspace=3\baselineskip,
		frametitleaboveskip=5em,
		innerrightmargin=5pt
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-2em}
	{\captionof{figure}{\normalfont \TitleCaption}\label{\TitleLabel}}
	%\medskip
	\vspace{-2mm}
}

%------------------------------------------------------------------------------
% Box Environments without embossed title
%------------------------------------------------------------------------------

\newenvironment{mysystembox}[3]
{\begin{titlebox*}{Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mygsystembox}[3]
{\begin{titlebox*}{Global Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myprotocolbox}[3]
{\begin{titlebox*}{Protocol \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myalgobox}[3]
{\begin{titlebox*}{Algorithm \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myreductionbox}[3]
{\begin{titlebox*}{Reduction \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mygamebox}[3]
{\begin{titlebox*}{Game \normalfont #1}{mycommonbox}{gray}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mysimulatorbox}[3]
{\begin{titlebox*}{Simulator \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}
%-------------------------------------------------------------------------------


%------------------------------------------------------------------------------
% Full Width Environments without embossed title
%------------------------------------------------------------------------------

\newenvironment{mysystembox*}[3]
{\begin{strip}
		\vspace{\baselineskip}\begin{titlebox*}{Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mygsystembox*}[3]
{\begin{strip}
		\vspace{\baselineskip}\begin{titlebox*}{Global Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myprotocolbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Protocol \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myalgobox*}[3]
{\begin{strip}
		\begin{titlebox*}{Algorithm \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myreductionbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Reduction \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mygamebox*}[3]
{\begin{strip}
		\begin{titlebox*}{Game \normalfont #1}{mycommonbox}{gray}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mysimulatorbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Simulator \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}






%-------------------------------------------------------------------------------
% Basic protocol box without Algohead NDSS
%-------------------------------------------------------------------------------
%Basic box structure with title box
\newenvironment{mytbox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.8\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1.5em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	%\smallskip
	\vspace{-2mm}
}

\newenvironment{mytsplitbox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.8\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-0.5em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	%\smallskip
	\vspace{-2mm}
}

\newenvironment{mypbox}[3]
{\begin{mytbox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{mytbox}}

\newenvironment{mypsplitbox}[3]
{\begin{mytsplitbox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{mytsplitbox}}











%-------------------------------------------------------------------------------
% Macros used for the examples
%-------------------------------------------------------------------------------

%----- Algorithm Environment ---------------------------------------------------
%Header for Algorithms/Functionalities
\newcommand{\algoHead}[1]{\vspace{0.2em} \underline{\textbf{#1}} \vspace{0.3em}}
\newcommand{\algoHeadN}[1]{\vspace{-1em} \underline{\textbf{#1}} \vspace{0.2em}}
\newcommand{\algoHeadExt}[2]{\vspace{0.2em} \underline{\textbf{#1} #2} \vspace{0.3em}}

%Multiline Algo-States
\makeatletter
\algnewcommand{\ExtendedState}[1]{\State
	\parbox[t]{\dimexpr\linewidth-\ALG@thistlm}{\hangindent=\algorithmicindent\strut\hangafter=3#1\strut}}
\makeatother

%Algorithms States
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

%Algo Comments
\algrenewcommand{\algorithmiccomment}[1]{{\color{gray}// #1}}

%  Font and Notation
%-------------------------------------------------------------------------------
\newcommand{\xmath}[1]{\ensuremath{#1}\xspace}

\newcommand{\command}[1]{\xmath{\textsc{#1}}}
\newcommand{\algorithm}[1]{\xmath{\mathsf{#1}}}
\newcommand{\variable}[1]{\xmath{\mathtt{#1}}}
\newcommand{\parameter}[1]{\xmath{\mathtt{#1}}}

%Nice empty set
\let\oldemptyset\emptyset
\let\emptyset\varnothing

%Functionalities
\newcommand{\Func}[1][\relax]{\xmath{\mathcal{F}_{\textsc{#1}}}}
%-------------------------------------------------------------------------------
